Massive star formation in Wolf-Rayet galaxies: II. Optical spectroscopy results

(Abridged) We have performed a comprehensive multiwavelength analysis of a sample of 20 starburst galaxies that show the presence of a substantial population of very young massive stars. In this paper, the second of the series, we present the results of the analysis of long-slit intermediate-resolution spectroscopy of star-formation bursts for 16 galaxies of our sample. We study the spatial localization of the WR stars in each galaxy. We analyze the excitation mechanism and derive the reddening coefficient, physical conditions and chemical abundances of the ionized gas. We study the kinematics of the ionized gas to check the rotation/turbulence pattern of each system. When possible, tentative estimates of the Keplerian mass of the galaxies have been calculated. Our analysis has revealed that a substantial fraction of the galaxies show evidences of perturbed kinematics. With respect to the results found in individual galaxies, we remark the detection of objects with different metallicity and decoupled kinematics in Haro 15 and Mkn 1199, the finding of evidences of tidal streams in IRAS 08208+2816, Tol 9 and perhaps in SBS 1319+579, and the development of a merging process in SBS 0926+606 A and in Tol 1457-262. All these results reinforce the hypothesis that interactions with or between dwarf objects is a very important mechanism in the triggering of massive star formation in starburst galaxies, specially in dwarf ones. It must be highlighted that only deep and very detailed observationscan provide clear evidences that these subtle interaction processes are taking place.

==> MSFinWRG_II_bibliography.tex <==

\begin{thebibliography}{}

\scriptsize{
%\usepackage{natbib}
%\bibpunct{(}{)}{;}{a}{}{,}

\bibitem[\protect\citeauthoryear{Abbott}{Abbott}{1982}]{Abbott82}	
Abbott, D.~C. 1982, ApJ, 263, 723 
\bibitem[\protect\citeauthoryear{Asplund, Grevesse \& Sauval}{Asplund et al.}{2005}]{ASP05}
Asplund, M., Grevesse, N. \& Sauval, A. J. 2005, in ASP Conf. Ser. 335, \emph{Cosmic Abundances as Records of Stellar Evolution and Nucleosynthesis}, ed. F.N. Bash \& T.G. Barnes (San Francisco: ASP), 25

\bibitem[\protect\citeauthoryear{Barnes et al.}{Barnes et al.}{2002}]{Barnes02}
Barnes, D.G. et al. 2001, MNRAS, 322, 486
\bibitem[\protect\citeauthoryear{Benjamin et al.}{Benjamin, Skillman \& Smits}{2002}]{B02}
Benjamin, R.A., Skillman, E.D. \& Smits, D.P. 2002, \apj,, 569, 288
\bibitem[\protect\citeauthoryear{Bettoni et al.}{Bettoni, Galleta \& Garc\'{\i}a-Murillo}{2003}]{Bettoni03}
Bettoni, D., Galleta, G. \& Garc\'{\i}a-Murillo, S. 2003, A\&A, 405, 5 
\bibitem[\protect\citeauthoryear{Buckalew et al.}{Buckalew, Kobulnicky \& Dufour}{2005}]{Buckalew05}
Buckalew, B.A., Kobulnicky, H.A. \& Dufour, R.J. 2005, ApJS, 157, 30

\bibitem[\protect\citeauthoryear{Campbell et al.}{Campbell, Terlevich \& Melnick}{1986}]{CTM86}
Campbell, A.W., Terlevich, R., \& Melnick, J. 1986, MNRAS, 223, 811
\bibitem[\protect\citeauthoryear{Cannon et al.}{Cannon et al.}{2004}]{CSK04}
Cannon, J.M., Skillman, E.D., Kunth, D., Leitherer, C., Mas-Hesse, M., \"Ostlin, M. \& Petrosian, A. 2004, ApJ, 608, 768
\bibitem[\protect\citeauthoryear{Cardelli et al.}{Cardelli, Clayton \& Mathis}{1989}]{Cardelli89}
Cardelli, J.~A., Clayton, G.~C. \& Mathis J.~S. 1989, ApJ, 345, 245
\bibitem[\protect\citeauthoryear{Conti}{Conti}{1976}]{Conti76} 
Conti, P.S., 1976,  MSRSL, 9, 193
\bibitem[\protect\citeauthoryear{Conti}{Conti}{1991}]{C91} 
Conti, P.S., 1991, \apj, 377, 115
\bibitem[\protect\citeauthoryear{Contini}{Contini}{1996}]{Contini96}
Contini, T. 1996, \emph{Liege International Astrophysical Colloquia 33: Wolf-Rayet stars in the framework of stellar evolution}, Liege: Universite de %%@
Liege, Institut d'Astrophysique, Edited by J.M. Vreux, A. Detal, D. Fraipont-Caro, E. Gosset, and G. Rauw, p.619

\bibitem[\protect\citeauthoryear{Dahlem et al.}{Dahlem et al.}{2005}]{Dahlem05}
Dahlem, M., Ehle, M., Ryder, S.~D., Vlaji{\'c}, M. \& Haynes, R.~F.\ 2005, \aap, 432, 475 
\bibitem[\protect\citeauthoryear{Denicol\'o et al.}{Denicol\'o, Terlevich \& Terlevich}{2002}]{D02}
Denicol\'o, G., Terlevich, R. \& Terlevich, E. 2002, \mnras, 330, 69
\bibitem[\protect\citeauthoryear{Dopita et al.}{Dopita et al.}{2000}]{Do00}
Dopita, M.A., Kewley, L. J., Heisler, C.A. \& Sutherland, R.S. 2000, \apj, 542, 224

\bibitem[\protect\citeauthoryear{Esteban et al.}{Esteban et al.}{2004}]{Est04}
Esteban, C., Peimbert, M., Garc\'{\i}a-Rojas, J., Ruiz, M. T., Peimbert, A. \& Rodr\'{\i}guez, M., 2004, \mnras, 355, 229

\bibitem[\protect\citeauthoryear{Fernandes et al.}{Fernandes et al.}{2004}]{FCCG04}
Fernandes, I.F., de Carvalho, R., Contini, T. \& Gal, R.R. 2004, MNRAS 355, 728
\bibitem[\protect\citeauthoryear{Fioc \& Rocca-Volmerange}{Fioc \& Rocca-Volmerange}{1997}]{PEGASE97}
Fioc, M. \& Rocca-Volmerange, B. 1997, A\&A 326, 950
\bibitem[\protect\citeauthoryear{French}{French}{1980}]{French80}
French, H.~B. 1980, \apj, 240, 41

\bibitem[\protect\citeauthoryear{Gallego et al.}{Gallego et al.}{1997}]{Gallego97}
Gallego, J.;,Zamorano, J., Rego, M. \& Vitores, A.G. 1997, ApJ, 475, 502
\bibitem[\protect\citeauthoryear{Garc\'{\i}a-Rojas et al.}{Garc\'{\i}a-Rojas et al.}{2004}]{GRE04}
Garc\'{\i}a-Rojas, J., Esteban, C., Peimbert, M., Rodr\'{\i}guez, M., Ruiz, M. T., \& Peimbert, A. 2004, \apjs, 153, 501
\bibitem[\protect\citeauthoryear{Garnett}{Garnett}{1992}]{G92}
Garnett, D.R. 1992, AJ, 103, 1330
\bibitem[\protect\citeauthoryear{Garnett et al.}{Garnett et al.}{1991}]{Garnett91}
Garnett, D.R., Kennicutt, R.~C.Jr., Chu, Y.-H. \& Skillman E.~D. 1991, ApJ, 373, 458 
\bibitem[\protect\citeauthoryear{Garnett}{Garnett}{2004}]{G04}
Garnett, D.R. 2003, lectures on \emph{Cosmochemistry: The melting pot of the elements}. XIII Canary Islands Winter School of Astrophysics, Puerto de la Cruz, Tenerife, Spain, November 19-30, 2001, edited by C. Esteban, R. J. Garc\'{\i}a L\'opez, A. Herrero, F. S\'anchez. Cambridge contemporary astrophysics. Cambridge, UK: Cambridge University Press, ISBN 0-521-82768-X, 2004, p. 171
\bibitem[\protect\citeauthoryear{Gordon \& Gottesman}{Gordon \& Gottesman}{1981}]{GG81}
Gordon, D. \& Gottesman, S.T. 1981, AJ, 86, 161
\bibitem[\protect\citeauthoryear{Guseva et al.}{Guseva, Izotov \& Thuan}{2000}]{GIT00}
Guseva, N., Izotov, Y. I. \& Thuan, T.X. 2000, ApJ, 531, 776
\bibitem[\protect\citeauthoryear{Guseva et al.}{Guseva et al.}(2001)]{GIP01}
Guseva, N.G., Izotov, Y.I., Papaderos, P., Chaffee, F.H., Foltz, C.B., Green, R.F., Thuan, T.X., Fricke, K.L. \& Noeske, K.G. 2001, A\&A, 378, 756
\bibitem[\protect\citeauthoryear{Guseva et al.}{Guseva et al.}{2003}]{Guseva03}
Guseva, N.G., Papaderos, P., Izotov, Y.I., Green, R.F., Fricke, K.J., Thuan, T.X. \& Noeske, K.G. 2003, A\&A, 407, 105


\bibitem[\protect\citeauthoryear{Hjorth et al.}{Hjorth et al.}{2003}]{Hjorth03}
Hjorth J., et al. 2003, Nature, 423, 847 
\bibitem[\protect\citeauthoryear{Huang et al.}{Huang et al.}{1999}]{HGJL99}
Huang, J.H., Gu, Q.S., Ji,L., Li, W.D., Wei, J.Y. \& Zheng, W. 1999, ApJ 513, 215 
\bibitem[\protect\citeauthoryear{Huchtmeier et al.}{Huchtmeier et al.}{1995}]{HSH95}
Huchtmeier, W.K., Sage, L.J. \& Henkel, C. 1995, A\&A, 300, 675
\bibitem[\protect\citeauthoryear{Huchtmeier et al.}{Huchtmeier, Krishna \& Petrosian}{2005}]{HKP05}
Huchtmeier, W.~K., Krishna, G. \& Petrosian, A.\ 2005, \aap, 434, 887 
\bibitem[\protect\citeauthoryear{Huchtmeier et al.}{Huchtmeier et al.}{2007}]{HPKK07}
Huchtmeier, W.~K., Petrosian, A., Krishna, G. \& Kunth, D. 2007, A\&A, 462, 919
\bibitem[\protect\citeauthoryear{Hunter \& Gallagher}{Hunter \& Gallagher}{1985}]{HG85}
Hunter, D.A. \& Gallagher, J.S., 1985, AJ, 90, 1457

\bibitem[\protect\citeauthoryear{Izotov et al.}{Izotov et al.}{1991}]{Izotov91}
Izotov, Y.I., Guseva, N.G., Lipovetskii, V.A., Kniazev, A.Y. \& Stepanian, J.A. 1991, A\&A, 247, 303
\bibitem[\protect\citeauthoryear{Izotov et al.}{Izotov, Thuan, \& Lipovetski}{1994}]{ITL94}
Izotov, Y.I., Thuan, T.X., \& Lipovetski, 1994, ApJ, 435, 647
\bibitem[\protect\citeauthoryear{Izotov et al.}{Izotov, Thuan \& Lipovetski}{1997}]{ITL97}
Izotov, Y.I., Thuan, T.X., \& Lipovetski, 1997, ApJS, 108, 1
%\bibitem[\protect\citeauthoryear{Izotov et al.}{Izotov et al.}{1997}]{Izotov97}
%Izotov, Y.~I., Foltz, C.~B., Green, R.~F., Guseva, N.~G. \& Thuan T.~X., 1997, ApJ, 487, L37 
\bibitem[\protect\citeauthoryear{Izotov \& Thuan}{Izotov \& Thuan}{1998}]{IT98}
Izotov, Y.I. \& Thuan, T.X., 1998, \apj, 500, 188
\bibitem[\protect\citeauthoryear{Izotov \& Thuan}{Izotov \& Thuan}{1999}]{IT99}
Izotov, Y.I. \& Thuan, T.X. 1999, ApJ, 511, 639
%\bibitem[\protect\citeauthoryear{Izotov et al.}{Izotov et al.}{1999}]{Izotov99}
%Izotov, Y.~I., Chaffee, F.~H., Foltz, C.~B., Green, R.~F., Guseva, N.~G. \& Thuan T.~X. 1999, ApJ, 527, 757
\bibitem[\protect\citeauthoryear{Izotov \& Thuan}{Izotov \& Thuan}{2004}]{IT04}
Izotov, Y.I. \& Thuan, T.X. 2004, ApJ, 616, 768
%\bibitem[\protect\citeauthoryear{Izotov et al.}{Izotov et al.}{2004}]{IPG04}
%Izotov, Y.I., Papaderos, P., Guseva, N.G., Fricke, K.J. \& Thuan, T.X. 2004, A\&A 421, 539



\bibitem[\protect\citeauthoryear{Kewley et al.}{Kewley et al.}{2001}]{KD01}
Kewley, L.J., Dopita, M.A., Sutherland, R.S., Heisler, C.A. \& Trevena, J. 2001, \apjs, 556, 121
\bibitem[\protect\citeauthoryear{Kobulnicky \& Skillman}{Kobulnicky \& Skillman}{1996}]{KS96}
Kobulnicky, H.A, \& Skillman, E.D. 1996, ApJ, 471, 211
\bibitem[\protect\citeauthoryear{Kobulnicky \& Skillman}{Kobulnicky \& Skillman}{2008}]{KS08}
Kobulnicky, H.A, \& Skillman, E.D. 2008, AJ, 135, 527
\bibitem[\protect\citeauthoryear{Kong et al.}{Kong et al.}{2002}]{Kong02}
Kong, X., Cheng, F.~Z., Weiss, A. \& Charlot, S.\ 2002, \aap, 396, 503
\bibitem[\protect\citeauthoryear{Koribalski}{Koribalski}{2008}]{Koribalski08}
Koribalski, B.S. 2008, proceedings of \emph{Galaxies in the Local Volume} conference, Springer, p.41
\bibitem[\protect\citeauthoryear{Kovo \& Contini}{Kovo \& Contini}{1999}]{KovoContini99}
Kovo, O. \& Contini, T. 1999, in \emph{Wolf-Rayet Phenomena in Massive Stars and Starburst Galaxies. Proceedings of the 193rd symposium of the International Astronomical Union held in Puerto Vallarta, Mexico, 3-7 November 1998}. Edited by Karel A. van der Hucht, Gloria Koenigsberger, and Philippe R. J. Eenens. San Francisco, Calif. : Astronomical Society of the Pacific, p.604
\bibitem[\protect\citeauthoryear{Kniazev et al.}{Kniazev et al.}{2004}]{Kniazev04}
Kniazev, A.Y., Pustilnik, S.A., Grebel, E.K., Lee., H. \& Pramsku, A.G. 2004, ApJS, 153, 429
\bibitem[\protect\citeauthoryear{Kunth \& Joubert}{Kunth \& Joubert}{1985}]{KJ85}
Kunth, D. \& Joubert, M. 1985, A\&A, 142, 411 
\bibitem[\protect\citeauthoryear{Kunth \& Schild}{Kunth \& Schild}{1986}]{KS86}
Kunth, D. \& Schild, H. 1986, A\&A, 169, 71 

\bibitem[\protect\citeauthoryear{Lauberts \& Valentijn}{Lauberts \& Valentijn}{1989}]{Lauberts89} 
Lauberts, A. \& Valentijn, E.A. 1989, \emph{The surface photometry catalogue of the ESO-Uppsala galaxies}, Garching: European Southern Observatory (ESO) 
\bibitem[\protect\citeauthoryear{Lee et al.}{Lee, Salzer \& Melbourne}{2004}]{Lee04}
Lee, J.C., Salzer J.J. \& Melbourne, J. 2004, ApJ, 616, 752L
\bibitem[\protect\citeauthoryear{Leitherer et al.}{Leitherer et al.}{1999}]{L99}
Leitherer, C., Schaerer, D., Goldader, J.D., Gonz\'alez-Delgado, R.M., Robert, C., Kune, D.F., de Mello, D.F., Devost, D. \& Heckman, T.M. 1999, ApJS, %%@
123, 3 (\emph{STARBURST~99})
\bibitem[L\'opez-S\'anchez(2006)]{LS06}
L\'opez-S\'anchez, \'A.R. 2006, PhD Thesis, Universidad de la Laguna (Tenerife, Spain)
%\bibitem[L\'opez-S\'anchez \& Esteban(2003)]{LSE03}
%L\'opez-S\'anchez, \'A.R. \& Esteban, 2003, Rev. Mex. Astron. Astrofis. Conf. Ser., 18, 48
\bibitem[L\'opez-S\'anchez et al.(2004a)]{LSER04a}
L\'opez-S\'anchez, \'A.R., Esteban, C. \& Rodr\'{\i}guez, M. 2004a, ApJS, 153, 243
\bibitem[L\'opez-S\'anchez et al.(2004b)]{LSER04b}
L\'opez-S\'anchez, \'A.R., Esteban, C. \& Rodr\'{\i}guez, M. 2004b, A\&A 428,445
\bibitem[\protect\citeauthoryear{L\'opez-S\'anchez et al.}{L\'opez-S\'anchez, Esteban \& Garc\'{\i}a-Rojas}{2006}]{LSEGR06}
L\'opez-S\'anchez, \'A.R., Esteban, C. \& Garc\'{\i}a-Rojas, J. 2006, A\&A, 449, 997
\bibitem[\protect\citeauthoryear{L\'opez-S\'anchez et al.}{L\'opez-S\'anchez et al.}{2007}]{LSEGRPR07}
L\'opez-S\'anchez, \'A.R., Esteban, C., Garc\'{\i}a-Rojas, J., Peimbert, M. \& Rodr\'{\i}guez, M. 2007, ApJ, 656, 168
\bibitem[\protect\citeauthoryear{L\'opez-S\'anchez et al.}{L\'opez-S\'anchez et al.}{2008}]{LS08a}
L\'opez-S\'anchez, \'A.R., Koribalski, B., Esteban, C. \& Garc\'{\i}a-Rojas, J. 2008, proceedings of \emph{Galaxies in the Local Volume}, Springer, p.53
\bibitem[\protect\citeauthoryear{L\'opez-S\'anchez \& Esteban}{L\'opez-S\'anchez \& Esteban}{2008}]{LSE08} 
L\'opez-S\'anchez, \'A.R. \& Esteban, C. 2008, A\&A, 491, 131, Paper~I
\bibitem[\protect\citeauthoryear{L\'opez-S\'anchez et al.}{L\'opez-S\'anchez et al.}{2009}]{LS09} 
L\'opez-S\'anchez, \'A.R. et al. 2009, in prep


\bibitem[\protect\citeauthoryear{Maeder}{Maeder}{1981}]{Maeder81}
Maeder, A. 1981, A\&A, 102, 401
\bibitem[\protect\citeauthoryear{Maeder}{Maeder}{1990}]{Maeder90}
Maeder, A. 1990, A\&AS, 84, 139 
\bibitem[\protect\citeauthoryear{Maeder}{Maeder}{1991}]{Maeder91}
Maeder, A. 1991, A\&A, 242, 93
\bibitem[\protect\citeauthoryear{Maeder \& Meynet}{Maeder \& Meynet}{1994}]{MaederMeynet94}
Maeder, A. \& Meynet, G. 1994, A\&A, 287, 803 
\bibitem[\protect\citeauthoryear{Melbourne \& Salzer}{Melbourne \& Salzer}{2002}]{Melbourne02}	
Melbourne, J. \& Salzer, J.J. 2002, AJ, 123, 2302
\bibitem[\protect\citeauthoryear{Melbourne et al.}{Melbourne et al.}{2004}]{Melbourne04}
Melbourne, J., Phillips, A., Salzer, J.J., Gronwall, C. \& Sarajedini, V.L. 2004, AJ, 127, 686
\bibitem[\protect\citeauthoryear{M\'endez \& Esteban}{M\'endez \& Esteban}{1997}]{ME97}
M\'endez, D.I. \& Esteban, C. 1997, ApJ, 488, 652
\bibitem[\protect\citeauthoryear{M\'endez \& Esteban}{M\'endez \& Esteban}{1999}]{ME99}
M\'endez, D.I. \& Esteban, C. 1999, AJ 118, 2733
\bibitem[\protect\citeauthoryear{Masegosa et al.}{Masegosa, Moles \& del Olmo}{1991}]{Masegosa91}
Masegosa, M., Moles, M. \& del Olmo, A. 1991, A\&A, 244, 273
\bibitem[\protect\citeauthoryear{Masegosa et al.}{Masegosa, Moles \& Campos-Aguilar}{1994}]{Masegosa94}
Masegosa, M., Moles, M. \& Campos-Aguilar, A. 1994, ApJ, 420, 576
\bibitem[\protect\citeauthoryear{Massey et al.}{Massey et al.}{1988}]{M88}
Massey P., Strobel K., Barnes J.V. \& Anderson E. 1988, ApJ 328, 315
\bibitem[\protect\citeauthoryear{Mazzarrella et al.}{Mazzarrella, Bothum \& Boronson}{1991}]{MBB91}
Mazzarella, J.M., Bothun, G.D. \& Boroson, T.A. 1991, AJ, 101, 2034 
\bibitem[\protect\citeauthoryear{Mazzarrella \& Boronson}{Mazzarrella \& Boronson}{1993}]{MB93}
Mazzarrella, J.M. \& Boronson, T.A. 1993, ApJS, 85, 27


\bibitem[\protect\citeauthoryear{Paturel et al.}{Paturel et al.}{2003}]{Paturel03}
Paturel, G., Theureau, G., Bottinelli, L., Gouguenheim, L., Coudreau-Durand, N., Hallet, N. \& Petit, C.\ 2003, \aap, 412, 57 
\bibitem[\protect\citeauthoryear{Peimbert \& Costero}{Peimbert \& Costero}{1969}]{PC69}
Peimbert, M. \& Costero, R. 1969, Bol. Obs. Tonantzintla y Tacubaya, 5, 3
\bibitem[\protect\citeauthoryear{Penston et al.}{Penston et al.}{1977}]{Penston97}
Penston, M.V., Fosbury, R.A.E., Ward, M.J. \& Wilson, A.S.\ 1977, \mnras, 180, 19 
\bibitem[\protect\citeauthoryear{Pe\~na et al.}{Pe\~na, Ruiz \& Maza}{1991}]{PenaRM91}	
Pe\~na, M., Ruiz, M.T. \& Maza, J. 1991, A\&A, 251, 417
\bibitem[\protect\citeauthoryear{P{\'e}rez-Montero \& D\'{\i}az}{P{\'e}rez-Montero \& D\'{\i}az}{2003}]{PerezMontero03}
P{\'e}rez-Montero, E. \& D{\'{\i}}az, A.~I.\ 2003, \mnras, 346, 105 
\bibitem[\protect\citeauthoryear{Perryman et al.}{Perryman et al.}{1982}]{Perryman82}
Perryman, M.A.C., Longair, M.S., Allington-Smith, J.R. \& Fielden, J. 1982, MNRAS, 201, 957
\bibitem[\protect\citeauthoryear{Pettini \& Pagel}{Pettini \& Pagel}{2004}]{PP04}
Pettini, M. \& Pagel, B.E.J. 2004, \mnras, 348, 59
\bibitem[\protect\citeauthoryear{Pilyugin}{Pilyugin}{2001a}]{P01a}
Pilyugin, L.S. 2001a, A\&A, 369, 594
\bibitem[\protect\citeauthoryear{Pilyugin}{Pilyugin}{2001b}]{P01b}
Pilyugin, L.S. 2001b, A\&A, 374, 412
\bibitem[\protect\citeauthoryear{Pindao}{Pindao}{1999}]{Pindao99}
Pindao, M.\ 1999, in \emph{IAU Symp.~193: Wolf-Rayet Phenomena in Massive Stars and Starburst Galaxies}, 193, 614
\bibitem[\protect\citeauthoryear{Pindao et al.}{Pindao et al.}{2002}]{PSGD02}
Pindao, M., Schaerer, D., Gonz\'alez-Delgado, R.M. \& Stasi\'nska, G. 2002, A\&A 394, 443
\bibitem[\protect\citeauthoryear{Pustilnik et al.}{Pustilnik et al.}{2002}]{Pustilnik02}
Pustilnik, S.~A., Martin, J.-M., Huchtmeier, W.~K., Brosch, N., Lipovetsky, V.~A. \& Richter, G.~M.\ 2002, \aap, 389, 405
\bibitem[\protect\citeauthoryear{Pustilnik et al.}{Pustilnik et al.}{2004}]{PKP04}
Pustilnik, S., Kniazev, A., Pramskij, A., Izotov, Y., Foltz, C., Brosch, N., Martin, J.-M. \& Ugryumov, A. 2004, A\&A 419, 469


\bibitem[\protect\citeauthoryear{Quinet}{Quinet}{1996}]{Q96}
Quinet, P. 1996, A\&AS, 116, 573

\bibitem[\protect\citeauthoryear{Rodr\'{\i}guez \& Rubin}{Rodr\'{\i}guez \& Rubin}{2005}]{RR05}
Rodr\'{\i}guez, M. \& Rubin, R.H. 2005, ApJ, 626, 900

\bibitem[\protect\citeauthoryear{Salzer et al.}{Salzer et al.}{2002}]{Salzer02}
Salzer, J.~J., Rosenberg, J.~L., Weisstein, E.~W., Mazzarella, J.~M. \& Bothun, G.~D. 2002, AJ, 124, 191
\bibitem[\protect\citeauthoryear{Sargent}{Sargent}{1970}]{Sargent70}
Sargent, W.L.W. 1970, ApJ, 160, 405
\bibitem[\protect\citeauthoryear{Schaerer et al.}{Schaerer, Contini \& Pindao}{1999}]{SCP99}
Schaerer, D., Contini, T. \& Pindao, M. 1999, A\&AS 136, 35
\bibitem[\protect\citeauthoryear{Schaerer et al.}{Schaerer et al.}{2000}]{SGIT00}
Schaerer, D., Guseva, N G., Izotov, Yu.I. \& Thuan, T.X. 2000, A\&A 362, 53
\bibitem[\protect\citeauthoryear{Schlegel et al.}{Schlegel, Finkbeiner \& Davis}{1998}]{SFD98}
Schlegel, D.J., Finkbeiner, D.P. \& Davis, M. 1998, ApJ, 500, 525
\bibitem[\protect\citeauthoryear{Shaw \& Dufour}{Shaw \& Dufour}{1995}]{SD95}
Shaw, R.A. \& Dufour, R.J. 1995, PASP, 107, 896
\bibitem[\protect\citeauthoryear{Shi et al.}{Shi et al.}{2005}]{Shi05} 
Shi, F., Kong, X., Li, C. \& Cheng, F.~Z.\ 2005, \aap, 437, 849
\bibitem[\protect\citeauthoryear{Skillman et al.}{Skillman et al.}{2003}]{SCM03}
Skillman, E.D., C\^ot\'e, S. \& Miller, B.W. 2003, AJ 125, 593
\bibitem[\protect\citeauthoryear{Smith et al.}{Smith, Shara \& Moffat}{1996}]{SSM96}
Smith, L.F., Shara, M.M. \& Moffat, A.F.J. 1996, MNRAS, 281, 163
\bibitem[\protect\citeauthoryear{Stasi\`nska}{Stasi\'nska}{1978}]{S78}
Stasi\'nska, G. 1978, A\&A, 66, 257
\bibitem[\protect\citeauthoryear{Storey \& Hummer}{Storey \& Hummer}{1995}]{SH95}
Storey, P.J. \& Hummer, D.G. 1995, MNRAS 272, 41

\bibitem[\protect\citeauthoryear{Terlevich et al.}{Terlevich et al.}{1991}]{Terlevich91}
Terlevich, R., Melnick, J., Masegosa, J., Moles, M. \& Copetti, M.V.F. 1991, A\&AS, 91, 285
\bibitem[\protect\citeauthoryear{Thuan et al.}{Thuan, Izotov \& Lipovetsky}{1995}]{TIL95}
Thuan, T.X., Izotov, Y.I., \& Lipovetsky, V.A. 1995, ApJ, 445, 108
\bibitem[\protect\citeauthoryear{Thuan, Izotov \& Foltz}{Thuan, Izotov \& Foltz}{1999}]{TIF99}
Thuan, T.X., Izotov Y.I. \& Foltz, C.B. 1999, ApJ, 525, 105
\bibitem[\protect\citeauthoryear{Thuan et al.}{Thuan et al}{1999}]{Thuan99}
Thuan, T.X., Lipovetski, V.A., Martin, J.-M. \& Pustilnik, S.A. 1999 A\&ASS, 139, 1


\bibitem[\protect\citeauthoryear{Vacca \& Conti}{Vacca \& Conti}{1992}]{VC92} 
Vacca, W.D. \& Conti, P.S., 1992, ApJ, 401, 543
\bibitem[\protect\citeauthoryear{Vaceli et al.}{Vaceli et al.}{1997}]{Va97}
Vaceli, M.S., Viegas, S.M., Gruenwald, R. \& De Souza, R.E. 1997, AJ, 114, 1345
\bibitem[\protect\citeauthoryear{van der Hucht}{van der Hucht}{2001}]{vH01}
van der Hucht, K.~A.\ 2001, \emph{7th Catalog of Galactic Wolf-Rayet stars},  NAR, 45, 135
\bibitem[\protect\citeauthoryear{van Zee et al.}{van Zee, Salzer \& Haynes}{1998}]{vZee98}
van Zee, L., Salzer, J.J. \&  Haynes, M.P. 1998, ApJ, 497, 1
\bibitem[\protect\citeauthoryear{V\'azquez \& Leitherer}{V\'azquez \& Leitherer}{2005}]{VL05}
V\'azquez, G.A. \& Leitherer, C. 2005, ApJ, 621, 695
\bibitem[\protect\citeauthoryear{Veilleux \& Osterbrock}{Veilleux \& Osterbrock}{1987}]{VO87}
Veilleux, S. \& Osterbrock, D.E. 1987, ApJS, 63 295

\bibitem[\protect\citeauthoryear{Westera et al.}{Westera et al.}{2004}]{Westera04}
Westera, P., Cuisinier, F., Telles, E. \& Kehrig, C. 2004, A\&A, 423, 133
\bibitem[\protect\citeauthoryear{Winkler}{Winkler}{1988}]{Winkler88}	
Winkler, H. 1988, MNRAS, 234, 703
\bibitem[\protect\citeauthoryear{Woodward}{Woodward}{1978}]{Woodward78}
Woodward P.~R. 1978, ARA\&A, 16, 555 
\bibitem[\protect\citeauthoryear{Woosley}{Woosley}{1993}]{Woosley93}
Woosley S.~E. 1993, ApJ, 405, 273 

\bibitem[\protect\citeauthoryear{Zasov et al.}{Zasov et al.}{2000}]{Zasov00}
Zasov, A.~V., Kniazev, A.~Y., Pustilnik, S.~A., Pramsky, A.~G., Burenkov, A.~N., Ugryumov, A.~V. \& Martin, J.-M.\ 2000, \aaps, 144, 429
\bibitem[\protect\citeauthoryear{Zhang}{Zhang}{1996}]{Z96}
Zhang, H. L. 1996, A\&AS, 119, 523




}

\bibliographystyle{aa} % style aa.bst
%\bibliography{angelitomosca.bib} % your references Yourfile.bib
\end{thebibliography}

